Enabling catalog simulations of transient and variable sources based on LSST cadence strategies

The Large Synoptic Survey Telescope (LSST) project will conduct a ten year multi-band survey starting in 2022. Observing strategies for this survey are being actively investigated, and the science capabilities can be best forecasted on the basis of simulated strategies from the LSST Operations Simulator (OpSim). OpSim simulates a stochastic realization of the sequence of LSST pointings over the survey duration, and is based on a model of the observatory (including telescope) and historical data of observational conditions. OpSim outputs contain a record of each simulated pointing of the survey along with a complete characterization of the pointing in terms of observing conditions, and some useful quantities derived from the characteristics of the pointing. Thus, each record can be efficiently used to derive the properties of observations of all astrophysical sources found in that pointing. However, in order to obtain the time series of observations (light curves) of a set of sources, it is often more convenient to compute all observations of an astrophysical source, and iterate over sources. In this document, we describe the open source python package OpSimSummary which allows for a convenient reordering. The objectives of this package are to provide users with an Application Programming Interface (API) for accessing all such observations and summarizing this information in the form intermediate data products usable by third party software such as SNANA, thereby also bridging the gap between official LSST products and pre-existing simulation codes.

==> simlib.tex <==
For a point source with intensity $\epsilon(\lambda)$ as a function of its wavelength $\lambda,$ the number of photons collected with an exposure time $T$ in a telescope with collecting area $A$ is given by:
\begin{equation}
C_{source} = \frac{AT}{h} \int_{0}^{\infty} F_{\nu}(\lambda) \lambda^{-1} d{\lambda} S^{Total}(\lambda)
%\label(eqn:source_counts_basic}
\end{equation}
where the flux $F_{\nu}(\lambda)$ is the frequency derivative of the intensity 
$F_{\nu}(\lambda) \equiv \frac{d\epsilon(\lambda)}{d\nu},$ 
while $S^{tot}(\lambda)$ is the total transmission due to the atmosphere, and the telescope system, and $h$ is the Planck constant. Similarly, using the intensity per unit area of the sky photons $b_{\nu}(\lambda),$ one can calculate the number of photons collected per pixel as
\begin{equation}
    c_{sky} = \frac{AT}{h} \int_{0}^{\infty} b_{\nu}(\lambda) \lambda^{-1} d{\lambda} S^{sys}(\lambda) p
\end{equation}
Using the definition of AB magnitudes, these can be written in the form:
\begin{eqnarray}
    C_{source} = \kappa 10^(-0.4 m) \\
    c_{sky} = \kappa \alpha \exp(-0.4 m_{sky})
\end{eqnarray} 
where $\kappa = 5445 (D/6.5m)^2 (T/30s) 10^{10} T_b$ and 
$\alpha = \Sigma_b$
\begin{equation}
    \mathrm{SNR} = \frac{C_{source}}{(C_{source} + N_{pix} \mathrm{pixArea} \times c_{sky})^{1/2}}
\end{equation}
Using the above equations,this gives us:
\begin{equation}
    \mathrm{SNR} = \frac{\kappa 10^{-0.4 m_{SNR}}}{(\kappa 10^{-0.4 m_{SNR}} + \alpha \kappa 10^{-0.4 m_{sky}})^{1/2}}
\end{equation}
    allowing one  to solve 
    \begin{equation}
        \kappa = \mathrm{SNR}^2 \left( 10^{0.4 m_{SNR}} + \alpha 10^{-0.4 (m_{sky} - 2 m_{SNR})} \right) 
\end{equation}
 

